Mobile Augmented Reality Framework with Fusional Localization and Pose Estimation

As a novel way of presenting information, augmented reality (AR) enables people to interact with the physical world in a direct and intuitive way. While there are some mobile AR products implemented with specific hardware at a high cost, the software approaches of AR implementation on mobile platforms(such as smartphones, tablet PC, etc.) are still far from practical use. GPS-based mobile AR systems usually perform poorly due to the inaccurate positioning in the indoor environment. Previous vision-based pose estimation methods need to continuously track predefined markers within a short distance, which greatly degrade user experience. This paper first conducts a comprehensive study of the state-of-the-art AR and localization systems on mobile platforms. Then, we propose an effective indoor mobile AR framework. In the framework, a fusional localization method and a new pose estimation implementation are developed to increase the overall matching rate and thus improving AR display accuracy. Experiments show that our framework has higher performance than approaches purely based on images or Wi-Fi signals. We achieve low average error distances (0.61-0.81m) and accurate matching rates (77%-82%) when the average sampling grid length is set to 0.5m.

==> related_work_section.tex <==

\section{Related work}

\subsection{Indoor Localization}
\textbf{Non-vision-based indoor localization methods.}
Methods simply based on these sensor inputs are proposed in some research, such as \cite{s24} and \cite{s6}. One of the most prominent approaches in WLAN-based indoors localization is Wi-Fi fingerprinting. Some researchers \cite{s8,s9} combine the inertia sensors and Wi-Fi fingerprints to do filtering (based on orientations and last positions) before comparing, which are known as pedestrian dead reckoning (PDR) methods. Machine learning models\cite{chriki2017svm,xie2016improved,cheng2018fast} can also be used in localization with Wi-Fi fingerprints.


\textbf{Vision-based indoor localization methods.} 
Marker-based methods (such as the indoor localization in ARQuack\cite{s12}) use pattern recognition to detect predefined markers for tracking. It is an efficient and mature way to locate as well as display AR information with little delay and power consumption, but it put strict limitations on the marker placement and observing distance.Semantics-based localization \cite{s29} uses semantic descriptors as features to locate users. Feature-based localization \cite{s26,s27} uses image features taken from the camera to retrieve possible images of indoor environments on servers. 

\subsection{Pose Estimation}

\textbf{Vision-based pose estimation methods.}
Vision-based pose estimation methods are widely studied and used. 1)POSIT has been used widely on many platforms, including smartphones. Some variants\cite{s34} or related systems\cite{s32,s33} have been proposed and the efficiency meets the expectations. 2)Image matching (such as \cite{s26,s27}) is most used to recognize fiducial markers in planar fiducial marker detection. Key point matching is applied with image features extracted from markers.3)Contour tracking\cite{s38} uses the contours of a 3D digital model to match the models. 

\textbf{Non-vision-based pose estimation methods.}
Most non-vision-based pose estimations use sensors like  GPS (such as the outdoor localization in ARQuack\cite{s12}), accelerators, compass and gyroscope to render virtual objects based on users' translations and rotations.  However, they can also be vibration-prone and less visually appealing since the alignments and poses of visual objects are entirely dependent on the hardware qualities which are usually poor. Besides, GPS-based AR systems will fail to provide precise localization information in indoor environments.

